Automatic Dialect Detection in Arabic Broadcast Speech

We investigate different approaches for dialect identification in Arabic broadcast speech, using phonetic, lexical features obtained from a speech recognition system, and acoustic features using the i-vector framework. We studied both generative and discriminate classifiers, and we combined these features using a multi-class Support Vector Machine (SVM). We validated our results on an Arabic/English language identification task, with an accuracy of 100%. We used these features in a binary classifier to discriminate between Modern Standard Arabic (MSA) and Dialectal Arabic, with an accuracy of 100%. We further report results using the proposed method to discriminate between the five most widely used dialects of Arabic: namely Egyptian, Gulf, Levantine, North African, and MSA, with an accuracy of 52%. We discuss dialect identification errors in the context of dialect code-switching between Dialectal Arabic and MSA, and compare the error pattern between manually labeled data, and the output from our classifier. We also release the train and test data as standard corpus for dialect identification.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> classifiers.tex <==
\label{sec:classifier}
\subsection{Generative Model}
\subsubsection{Trigram Langugage Modelling}
A different trigram model with Kneser-Ney smoothing is built for each dialect using the training set. The language model can be represented by equation~\ref{lm}.
\begin{equation}
  P(w_{1},w_{2},\ldots,w_{n})=\prod_{i=1}^{n} P(w_{i} | w_{i-2},w_{i-1}) \label{lm}
\end{equation}
where, $w_{0}=w_{-1}=*$. $*$ is a special start symbol~\cite{Collins}.

Given a test utterance and its correponding word sequence, perplexity of the word sequence is calculated using each dialectal language model. The one that gives the lowest perplexity is chosen as the dialect of the test utterance.

\subsubsection{Naive Bayes}
We use a standard Naive Bayes classifier as used in text classification, where the feature vector, $x$ is assumed to be made up of discrete features, where each element $x_{i}$, is either $0$ or $1$, indicating the presence or absence of the word at dictionary index $i$. The feature vector dimensionality is equal to the vocabulary size. The model parameters are estimated via Maximum Likelihood Estimation using the training set. For more details and the likelihhod equation, the reader is referred to an excellent tutorial~\cite{Ng}.

Given a test feature vector, $x^{*}$, and the model parameters $\theta$, the class $c$ (dialect) that $x^{*}$ belongs to is given by:

\begin{equation}
  c=\argmax_{c} p(x^{*}|y=c,\theta)p(y=c)
\end{equation}

\subsection{Discriminative Classifiers}
\subsubsection{Maximum Entropy}
Maximum Entropy classification is another popular technique used in document classiciation and we use the same technique for utterance classification to determine the dialect of the utterance. For the lack of space we refer the reader to the seminal work done by~\cite{Nigam}.

\subsubsection{Linear SVM}
We used a multi-class kernel classifier using regularization parameters to trade off margin size and training error. Given a test utterance the SVM otputs a score for each dialect, and the dialect that is given the highest score is chosen as the dialect of the utterance


==> code-switching.tex <==
\label{sec:code-switching}
 The detailed error pattern and confusion matrix in Table~\ref{tab:best_system} shows that GLF and LAV very often got confused more than any other pair. We hypothesise that this is related to the greater lexical similarity between LAV and GLF, illustrated in Table~\ref{tab:lexical_difference}.  % We also note that MSA significantly outperforms the rest of dialectal Arabic in classification.  We believe that this is because the acoustic training data mainly comprises MSA data, which can be considered to tune lexical and phonetic features to MSA.

Speaker linking information in the test set has been calculated using~\cite{meignier2010lium}. In our experiments, it is assumed that each segment (belonging to one speaker) is one dialect and speakers will not switch between dialects without reasonable silence (chosen to be 300ms), which seems to be a rather naive assumption. The authors have plans to visit a more fine-grained dialect diarization in the future~\cite{Wu2015} %This assumption has been accepted by the crowdsource community\footnote{It can be argued that in dialectal Arabic speakers can switch between MSA and dialects without silence. The authors have plans to visit a more fine-grained dialect diarization in the future.}.
  \begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.25]{DialectDetectionSpace}
    \caption{LDA projection for All Dialectal Features.}
    \label{fig:best_system}
  \end{figure}
%\subsection{MSA and Dialectal Arabic Code-Switching}
As shown in Figure~\ref{fig:best_system}, we see two dialects LAV and GLF overlap more with MSA compared to NOR or EGY. The crowdsourcing experiment~\cite{samn2015crowdsource} also provided manual annotations of 200 speech segments from each dialect as well as MSA. The input comprises speech segments from speakers with known dialect, and the judges chose freely which dialect each speech segment belongs to. For example, there are 200 samples from potential Gulf speakers. After labeling them, there are 106 segments labeled to be MSA, 82 validated as GLF, and 8 LAV, and 4 segments were not identified with enough confidence to be considered.  The results are shown in Table~\ref{tab:expansion2}, where it can be observed that code-switching happens most often between GLF/MSA and LAV/MSA. It is very interesting to observe that potential GLF speakers in this sample speak MSA more than 50\% of the time, and for LAV speakers, nearly 40\% of their speech is in MSA. This summary could explain that the overlap for MSA, GLF and LAV in Figure~\ref{fig:best_system} mainly occurs in code-switching rather than just an error in dialect identification.

Arabic native speakers will often speak only one dialect but will in many cases switch to MSA when using formal speech. It is therefore reasonable to assume that a detected switch between dialects is likely to be an error. This is a challenge for a subjective human judge according to our finding in some of the crowdsource feedback. %, where the decision is forced between closed dialects such as GLF or LAV based on the acoustics alone.


\begin{table}[ht!]
\centering
\begin{tabular}{p{2.4cm} | r | r | r | r |r}
  \hline
  Expected Dialect & EGY & GLF & LAV & NOR & MSA\\ \hline
  EGY &65\%\cellcolor[gray]{0.9}&&&&32\%\\ \hline
   GLF & &41\%&4\%&&53\%\cellcolor[gray]{0.9}\\ \hline
   LAV &1\%& 1\%& 53\%\cellcolor[gray]{0.9}&&39\%\\ \hline
   NOR & 1\%& &&69\%\cellcolor[gray]{0.9}&28\%\\
  \hline
\end{tabular}
\caption{Expected dialect of the file based on expansion at a 75\% confidence threshold from initial annotation by actual results}
\label{tab:expansion2}
\end{table}


==> dialect_challenges.tex <==
\label{sec:dialect_challenges}
 
An objective comparison of the varieties of Arabic dialects, especially at the edges of the Arabic-speaking area, might lead someone to conclude that they were historically related, but are synchronically and mutually unintelligible languages like English and Dutch; normal vernacular can be difficult to understand across different Arabic Dialects~\cite{holes2004modern}. 

%This inspired us to look at speech DID  in Arabic dialects similarly to LID task in other languages, which makes this task unique and interesting in itself. One can look at some examples across different dialects, as well as in MSA that shows significant lexical variates as shown in Table~\ref{tab:lexical_difference}.
Arabic dialects are thus sufficiently distinctive, that it is reasonable to regard the DID task in Arabic as similar to the LID task in other languages.  Table~\ref{tab:lexical_difference} shows examples of two phrases across some different dialects, as well as MSA, and makes clear the lexical variation, which is  greater than when comparing differences across dialects in many other languages such as English.    
 
\FloatBarrier   
\begin{table}[ht]
\label{lexicalExamples}
\caption{Lexical examples showed in Arabic and Buckwalter format}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
         & EGY     & GLF    & LAV           & MSA      & NOR     & English Translation \\ \hline
Example1 &   \begin{tabular}[x]{@{}c@{}} \novocalize \RL{AzAyk} \\AzAYk\end{tabular}                                                               & 
\begin{tabular}[x]{@{}c@{}} \novocalize \RL{A^slwnk} \\ A\$lwnk\end{tabular}                             & \begin{tabular}[x]{@{}c@{}} \novocalize \RL{A^slwnk / kyfk} \\ kyfk / A\$lwnk \end{tabular}      & \begin{tabular}[x]{@{}c@{}} \novocalize \RL{kyf .hAlk} \\ kyf HAlk\end{tabular}                            &  \begin{tabular}[x]{@{}c@{}} \novocalize \RL{wA^s rAk} \\ wA\$ rAk\end{tabular}                          & 
How are you?        \\ \hline

Example2 &   \begin{tabular}[x]{@{}c@{}} \novocalize \RL{Ant fen} \\Ant fyn\end{tabular}       &  
\begin{tabular}[x]{@{}c@{}} \novocalize \RL{wynk} \\wynk\end{tabular}                       				  & 
\begin{tabular}[x]{@{}c@{}} \novocalize \RL{wynk} \\wynk\end{tabular}                        				  & 
\begin{tabular}[x]{@{}c@{}} \novocalize \RL{Ayn Ant} \\ Ayn Ant\end{tabular}           					 &  
\begin{tabular}[x]{@{}c@{}} \novocalize \RL{wyn rAk} \\ wyn rAk\end{tabular}             				&
Where are you?        \\ \hline
\end{tabular}
}
\label{tab:lexical_difference}
\end{table}
\FloatBarrier

\noindent
%The two aforementioned examples in Table~\ref{tab:lexical_difference} show major lexical differences between Arabic dialects, and with MSA as well, %with an exception of LAV and GLF.
%clearly this is not the case in other languages such as when comparing American, British, and Australian English dialects. In this paper, when dialectal Arabic is mentioned, it does not include MSA. In this study, we depict lexical, phonetic, and acoustic features; namely four discriminative categories: phoneme sequence, phoneme duration, lexical, and acoustic features.



==> featureab.tex <==
\label{sec:fab}

